TrivialAugment: Tuning-free Yet State-of-the-Art Data Augmentation

Automatic augmentation methods have recently become a crucial pillar for strong model performance in vision tasks. While existing automatic augmentation methods need to trade off simplicity, cost and performance, we present a most simple baseline, TrivialAugment, that outperforms previous methods for almost free. TrivialAugment is parameter-free and only applies a single augmentation to each image. Thus, TrivialAugment's effectiveness is very unexpected to us and we performed very thorough experiments to study its performance. First, we compare TrivialAugment to previous state-of-the-art methods in a variety of image classification scenarios. Then, we perform multiple ablation studies with different augmentation spaces, augmentation methods and setups to understand the crucial requirements for its performance. Additionally, we provide a simple interface to facilitate the widespread adoption of automatic augmentation methods, as well as our full code base for reproducibility. Since our work reveals a stagnation in many parts of automatic augmentation research, we end with a short proposal of best practices for sustained future progress in automatic augmentation methods.

==> images/searchplot.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}
\scriptsize

\definecolor{color0}{rgb}{0.687392669486095,0.798284634115084,0.866250800973984}
\definecolor{color1}{rgb}{0.674295142893759,0.789216327053697,0.860442778418557}
\definecolor{color2}{rgb}{0.661197616301423,0.780148019992311,0.85463475586313}
\definecolor{color3}{rgb}{0.648100089709086,0.771079712930924,0.848826733307702}
\definecolor{color4}{rgb}{0.63500256311675,0.762011405869537,0.843018710752275}
\definecolor{color5}{rgb}{0.61863065487633,0.750676022042804,0.835758682557991}
\definecolor{color6}{rgb}{0.605533128283993,0.741607714981417,0.829950660002563}
\definecolor{color7}{rgb}{0.592435601691657,0.73253940792003,0.824142637447136}
\definecolor{color8}{rgb}{0.579338075099321,0.723471100858644,0.818334614891708}
\definecolor{color9}{rgb}{0.566240548506984,0.714402793797257,0.812526592336281}
\definecolor{color10}{rgb}{0.549868640266564,0.703067409970524,0.805266564141997}
\definecolor{color11}{rgb}{0.536771113674228,0.693999102909137,0.799458541586569}
\definecolor{color12}{rgb}{0.523673587081892,0.684930795847751,0.793650519031142}
\definecolor{color13}{rgb}{0.510576060489555,0.675862488786364,0.787842496475714}
\definecolor{color14}{rgb}{0.497478533897219,0.666794181724978,0.782034473920287}
\definecolor{color15}{rgb}{0.481106625656799,0.655458797898244,0.774774445726003}
\definecolor{color16}{rgb}{0.468009099064462,0.646390490836858,0.768966423170575}
\definecolor{color17}{rgb}{0.454911572472126,0.637322183775471,0.763158400615148}
\definecolor{color18}{rgb}{0.44181404587979,0.628253876714084,0.75735037805972}
\definecolor{color19}{rgb}{0.428716519287454,0.619185569652697,0.751542355504293}
\definecolor{color20}{rgb}{0.412344611047033,0.607850185825965,0.744282327310009}
\definecolor{color21}{rgb}{0.399247084454697,0.598781878764578,0.738474304754582}
\definecolor{color22}{rgb}{0.386149557862361,0.589713571703191,0.732666282199154}
\definecolor{color23}{rgb}{0.373052031270024,0.580645264641804,0.726858259643727}
\definecolor{color24}{rgb}{0.359954504677688,0.571576957580418,0.721050237088299}
\definecolor{color25}{rgb}{0.343582596437268,0.560241573753684,0.713790208894015}
\definecolor{color26}{rgb}{0.330485069844931,0.551173266692298,0.707982186338588}

\pgfplotsset{%
    width=1.\textwidth,
    height=.5\textwidth
}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={},%Augmentations},
xmin=-0.5, xmax=26.5,
xtick style={draw=none},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26},
xticklabel style = {rotate=90.0},
xticklabels={auto\_contrast,equalize,brightness,posterize,translate\_y,color,contrast,detail,flip\_lr,translate\_x,sharpen,solarize,sharpness,cutout,shear\_y,edge\_enhance,crop\_bilinear,shear\_x,contour,invert,min\_,median,max\_,rotate,flip\_ud,blur,gaussian},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymin=80.5, ymax=82.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0.4,80.7933333333333);
\draw[draw=none,fill=color1] (axis cs:0.6,0) rectangle (axis cs:1.4,81.0566666666667);
\draw[draw=none,fill=color2] (axis cs:1.6,0) rectangle (axis cs:2.4,81.1833333333333);
\draw[draw=none,fill=color3] (axis cs:2.6,0) rectangle (axis cs:3.4,80.9);
\draw[draw=none,fill=color4] (axis cs:3.6,0) rectangle (axis cs:4.4,81.12);
\draw[draw=none,fill=color5] (axis cs:4.6,0) rectangle (axis cs:5.4,81.6);
\draw[draw=none,fill=color6] (axis cs:5.6,0) rectangle (axis cs:6.4,81.2166666666667);
\draw[draw=none,fill=color7] (axis cs:6.6,0) rectangle (axis cs:7.4,81.39);
\draw[draw=none,fill=color8] (axis cs:7.6,0) rectangle (axis cs:8.4,81.3366666666667);
\draw[draw=none,fill=color9] (axis cs:8.6,0) rectangle (axis cs:9.4,81.4233333333333);
\draw[draw=none,fill=color10] (axis cs:9.6,0) rectangle (axis cs:10.4,81.77);
\draw[draw=none,fill=color11] (axis cs:10.6,0) rectangle (axis cs:11.4,82.03);
\draw[draw=none,fill=color12] (axis cs:11.6,0) rectangle (axis cs:12.4,82.0566666666667);
\draw[draw=none,fill=color13] (axis cs:12.6,0) rectangle (axis cs:13.4,81.9933333333333);
\draw[draw=none,fill=color14] (axis cs:13.6,0) rectangle (axis cs:14.4,82.0466666666667);
\draw[draw=none,fill=color15] (axis cs:14.6,0) rectangle (axis cs:15.4,81.7833333333333);
\draw[draw=none,fill=color16] (axis cs:15.6,0) rectangle (axis cs:16.4,82.1366666666667);
\draw[draw=none,fill=color17] (axis cs:16.6,0) rectangle (axis cs:17.4,81.91);
\draw[draw=none,fill=color18] (axis cs:17.6,0) rectangle (axis cs:18.4,81.68);
\draw[draw=none,fill=color19] (axis cs:18.6,0) rectangle (axis cs:19.4,81.68);
\draw[draw=none,fill=color20] (axis cs:19.6,0) rectangle (axis cs:20.4,81.3833333333333);
\draw[draw=none,fill=color21] (axis cs:20.6,0) rectangle (axis cs:21.4,81.5033333333333);
\draw[draw=none,fill=color22] (axis cs:21.6,0) rectangle (axis cs:22.4,81.3);
\draw[draw=none,fill=color23] (axis cs:22.6,0) rectangle (axis cs:23.4,81.1333333333333);
\draw[draw=none,fill=color24] (axis cs:23.6,0) rectangle (axis cs:24.4,81.96);
\draw[draw=none,fill=color25] (axis cs:24.6,0) rectangle (axis cs:25.4,81.4966666666667);
\draw[draw=none,fill=color26] (axis cs:25.6,0) rectangle (axis cs:26.4,81.18);
\addplot [line width=1.08pt, white!26!black]
table {%
0 80.68
0 80.94
};
\addplot [line width=1.08pt, white!26!black]
table {%
1 80.86
1 81.17
};
\addplot [line width=1.08pt, white!26!black]
table {%
2 80.8
2 81.42
};
\addplot [line width=1.08pt, white!26!black]
table {%
3 80.69
3 81.07
};
\addplot [line width=1.08pt, white!26!black]
table {%
4 81.01
4 81.29
};
\addplot [line width=1.08pt, white!26!black]
table {%
5 81.48
5 81.77
};
\addplot [line width=1.08pt, white!26!black]
table {%
6 81.06
6 81.41
};
\addplot [line width=1.08pt, white!26!black]
table {%
7 81.2433333333333
7 81.58
};
\addplot [line width=1.08pt, white!26!black]
table {%
8 81.25
8 81.44
};
\addplot [line width=1.08pt, white!26!black]
table {%
9 81.2
9 81.54
};
\addplot [line width=1.08pt, white!26!black]
table {%
10 81.51
10 82.03
};
\addplot [line width=1.08pt, white!26!black]
table {%
11 81.88
11 82.27
};
\addplot [line width=1.08pt, white!26!black]
table {%
12 81.73
12 82.42
};
\addplot [line width=1.08pt, white!26!black]
table {%
13 81.82
13 82.08
};
\addplot [line width=1.08pt, white!26!black]
table {%
14 81.85
14 82.18
};
\addplot [line width=1.08pt, white!26!black]
table {%
15 81.6
15 81.92
};
\addplot [line width=1.08pt, white!26!black]
table {%
16 81.9
16 82.26
};
\addplot [line width=1.08pt, white!26!black]
table {%
17 81.8
17 82.07
};
\addplot [line width=1.08pt, white!26!black]
table {%
18 81.64275
18 81.73
};
\addplot [line width=1.08pt, white!26!black]
table {%
19 81.27
19 81.9
};
\addplot [line width=1.08pt, white!26!black]
table {%
20 81.33
20 81.48
};
\addplot [line width=1.08pt, white!26!black]
table {%
21 81.33
21 81.67
};
\addplot [line width=1.08pt, white!26!black]
table {%
22 80.91
22 81.54
};
\addplot [line width=1.08pt, white!26!black]
table {%
23 80.97
23 81.22
};
\addplot [line width=1.08pt, white!26!black]
table {%
24 81.92
24 82
};
\addplot [line width=1.08pt, white!26!black]
table {%
25 81.37
25 81.74
};
\addplot [line width=1.08pt, white!26!black]
table {%
26 80.84
26 81.37
};
\end{axis}

\end{tikzpicture}


==> images/searchplot_cifar10.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}
\scriptsize

\definecolor{color0}{rgb}{0.687392669486095,0.798284634115084,0.866250800973984}
\definecolor{color1}{rgb}{0.674295142893759,0.789216327053697,0.860442778418557}
\definecolor{color2}{rgb}{0.661197616301423,0.780148019992311,0.85463475586313}
\definecolor{color3}{rgb}{0.648100089709086,0.771079712930924,0.848826733307702}
\definecolor{color4}{rgb}{0.63500256311675,0.762011405869537,0.843018710752275}
\definecolor{color5}{rgb}{0.61863065487633,0.750676022042804,0.835758682557991}
\definecolor{color6}{rgb}{0.605533128283993,0.741607714981417,0.829950660002563}
\definecolor{color7}{rgb}{0.592435601691657,0.73253940792003,0.824142637447136}
\definecolor{color8}{rgb}{0.579338075099321,0.723471100858644,0.818334614891708}
\definecolor{color9}{rgb}{0.566240548506984,0.714402793797257,0.812526592336281}
\definecolor{color10}{rgb}{0.549868640266564,0.703067409970524,0.805266564141997}
\definecolor{color11}{rgb}{0.536771113674228,0.693999102909137,0.799458541586569}
\definecolor{color12}{rgb}{0.523673587081892,0.684930795847751,0.793650519031142}
\definecolor{color13}{rgb}{0.510576060489555,0.675862488786364,0.787842496475714}
\definecolor{color14}{rgb}{0.497478533897219,0.666794181724978,0.782034473920287}
\definecolor{color15}{rgb}{0.481106625656799,0.655458797898244,0.774774445726003}
\definecolor{color16}{rgb}{0.468009099064462,0.646390490836858,0.768966423170575}
\definecolor{color17}{rgb}{0.454911572472126,0.637322183775471,0.763158400615148}
\definecolor{color18}{rgb}{0.44181404587979,0.628253876714084,0.75735037805972}
\definecolor{color19}{rgb}{0.428716519287454,0.619185569652697,0.751542355504293}
\definecolor{color20}{rgb}{0.412344611047033,0.607850185825965,0.744282327310009}
\definecolor{color21}{rgb}{0.399247084454697,0.598781878764578,0.738474304754582}
\definecolor{color22}{rgb}{0.386149557862361,0.589713571703191,0.732666282199154}
\definecolor{color23}{rgb}{0.373052031270024,0.580645264641804,0.726858259643727}
\definecolor{color24}{rgb}{0.359954504677688,0.571576957580418,0.721050237088299}
\definecolor{color25}{rgb}{0.343582596437268,0.560241573753684,0.713790208894015}
\definecolor{color26}{rgb}{0.330485069844931,0.551173266692298,0.707982186338588}

\pgfplotsset{%
    width=1.\textwidth,
    height=.5\textwidth
}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={},%Augmentations},
xmin=-0.5, xmax=26.5,
xtick style={draw=none},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26},
xticklabel style = {rotate=90.0},
xticklabels={equalize,contrast,sharpen,solarize,detail,sharpness,auto\_contrast,translate\_y,cutout,shear\_y,brightness,flip\_lr,color,crop\_bilinear,translate\_x,posterize,edge\_enhance,contour,min\_,shear\_x,max\_,rotate,invert,blur,median,gaussian,flip\_ud},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymin=96.7, ymax=97.45,
ytick style={color=black},
ytick={96.4,96.6,96.8,97,97.2,97.4,97.6},
yticklabels={96.4,96.6,96.8,97.0,97.2,97.4,97.6}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0.4,96.9633333333333);
\draw[draw=none,fill=color1] (axis cs:0.6,0) rectangle (axis cs:1.4,96.8166666666667);
\draw[draw=none,fill=color2] (axis cs:1.6,0) rectangle (axis cs:2.4,97.0133333333333);
\draw[draw=none,fill=color3] (axis cs:2.6,0) rectangle (axis cs:3.4,96.9833333333333);
\draw[draw=none,fill=color4] (axis cs:3.6,0) rectangle (axis cs:4.4,97.1);
\draw[draw=none,fill=color5] (axis cs:4.6,0) rectangle (axis cs:5.4,97.06);
\draw[draw=none,fill=color6] (axis cs:5.6,0) rectangle (axis cs:6.4,97.0833333333333);
\draw[draw=none,fill=color7] (axis cs:6.6,0) rectangle (axis cs:7.4,97.1666666666667);
\draw[draw=none,fill=color8] (axis cs:7.6,0) rectangle (axis cs:8.4,97.1266666666667);
\draw[draw=none,fill=color9] (axis cs:8.6,0) rectangle (axis cs:9.4,97.0733333333333);
\draw[draw=none,fill=color10] (axis cs:9.6,0) rectangle (axis cs:10.4,97.2333333333333);
\draw[draw=none,fill=color11] (axis cs:10.6,0) rectangle (axis cs:11.4,97.24);
\draw[draw=none,fill=color12] (axis cs:11.6,0) rectangle (axis cs:12.4,97.27);
\draw[draw=none,fill=color13] (axis cs:12.6,0) rectangle (axis cs:13.4,97.22);
\draw[draw=none,fill=color14] (axis cs:13.6,0) rectangle (axis cs:14.4,97.2833333333333);
\draw[draw=none,fill=color15] (axis cs:14.6,0) rectangle (axis cs:15.4,97.2433333333333);
\draw[draw=none,fill=color16] (axis cs:15.6,0) rectangle (axis cs:16.4,97.0733333333333);
\draw[draw=none,fill=color17] (axis cs:16.6,0) rectangle (axis cs:17.4,97.1966666666667);
\draw[draw=none,fill=color18] (axis cs:17.6,0) rectangle (axis cs:18.4,97.1133333333333);
\draw[draw=none,fill=color19] (axis cs:18.6,0) rectangle (axis cs:19.4,97.2733333333333);
\draw[draw=none,fill=color20] (axis cs:19.6,0) rectangle (axis cs:20.4,97.08);
\draw[draw=none,fill=color21] (axis cs:20.6,0) rectangle (axis cs:21.4,97.26);
\draw[draw=none,fill=color22] (axis cs:21.6,0) rectangle (axis cs:22.4,97.2);
\draw[draw=none,fill=color23] (axis cs:22.6,0) rectangle (axis cs:23.4,97.1333333333333);
\draw[draw=none,fill=color24] (axis cs:23.6,0) rectangle (axis cs:24.4,97.0233333333333);
\draw[draw=none,fill=color25] (axis cs:24.6,0) rectangle (axis cs:25.4,97.0266666666667);
\draw[draw=none,fill=color26] (axis cs:25.6,0) rectangle (axis cs:26.4,96.9133333333333);
\addplot [line width=1.08pt, white!26!black]
table {%
0 96.84
0 97.04
};
\addplot [line width=1.08pt, white!26!black]
table {%
1 96.76
1 96.89
};
\addplot [line width=1.08pt, white!26!black]
table {%
2 96.95
2 97.06
};
\addplot [line width=1.08pt, white!26!black]
table {%
3 96.89
3 97.15
};
\addplot [line width=1.08pt, white!26!black]
table {%
4 97.0865
4 97.12
};
\addplot [line width=1.08pt, white!26!black]
table {%
5 97.04
5 97.07
};
\addplot [line width=1.08pt, white!26!black]
table {%
6 97.08
6 97.09
};
\addplot [line width=1.08pt, white!26!black]
table {%
7 97.09
7 97.22
};
\addplot [line width=1.08pt, white!26!black]
table {%
8 97
8 97.2
};
\addplot [line width=1.08pt, white!26!black]
table {%
9 97.03
9 97.14
};
\addplot [line width=1.08pt, white!26!black]
table {%
10 97.19
10 97.29
};
\addplot [line width=1.08pt, white!26!black]
table {%
11 97.18
11 97.33
};
\addplot [line width=1.08pt, white!26!black]
table {%
12 97.2
12 97.39
};
\addplot [line width=1.08pt, white!26!black]
table {%
13 97.1633333333333
13 97.33
};
\addplot [line width=1.08pt, white!26!black]
table {%
14 97.19
14 97.34
};
\addplot [line width=1.08pt, white!26!black]
table {%
15 97.17
15 97.3045
};
\addplot [line width=1.08pt, white!26!black]
table {%
16 96.93
16 97.17
};
\addplot [line width=1.08pt, white!26!black]
table {%
17 97.11
17 97.27
};
\addplot [line width=1.08pt, white!26!black]
table {%
18 97.05
18 97.21
};
\addplot [line width=1.08pt, white!26!black]
table {%
19 97.18
19 97.4
};
\addplot [line width=1.08pt, white!26!black]
table {%
20 97
20 97.16
};
\addplot [line width=1.08pt, white!26!black]
table {%
21 97.18
21 97.37
};
\addplot [line width=1.08pt, white!26!black]
table {%
22 97.14
22 97.26
};
\addplot [line width=1.08pt, white!26!black]
table {%
23 97.04
23 97.19
};
\addplot [line width=1.08pt, white!26!black]
table {%
24 97
24 97.05
};
\addplot [line width=1.08pt, white!26!black]
table {%
25 96.93
25 97.15
};
\addplot [line width=1.08pt, white!26!black]
table {%
26 96.84
26 97.06
};
\end{axis}

\end{tikzpicture}


==> images/searchplot_old.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}


\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\scriptsize

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-1.74, xmax=27.74,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26},
xticklabel style = {rotate=90.0},
xticklabels={auto\_contrast,equalize,brightness,posterize,translate\_y,color,contrast,detail,flip\_lr,translate\_x,sharpen,solarize,sharpness,cutout,shear\_y,edge\_enhance,crop\_bilinear,shear\_x,contour,invert,min\_,median,max\_,rotate,flip\_ud,blur,gaussian},
y grid style={white!69.0196078431373!black},
ymin=80, ymax=82.5,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-0.4,0) rectangle (axis cs:0.4,80.7933333333333);
\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:1.4,81.0566666666667);
\draw[draw=none,fill=color0] (axis cs:1.6,0) rectangle (axis cs:2.4,81.1833333333333);
\draw[draw=none,fill=color0] (axis cs:2.6,0) rectangle (axis cs:3.4,80.9);
\draw[draw=none,fill=color0] (axis cs:3.6,0) rectangle (axis cs:4.4,81.12);
\draw[draw=none,fill=color0] (axis cs:4.6,0) rectangle (axis cs:5.4,81.6);
\draw[draw=none,fill=color0] (axis cs:5.6,0) rectangle (axis cs:6.4,81.2166666666667);
\draw[draw=none,fill=color0] (axis cs:6.6,0) rectangle (axis cs:7.4,81.39);
\draw[draw=none,fill=color0] (axis cs:7.6,0) rectangle (axis cs:8.4,81.3366666666667);
\draw[draw=none,fill=color0] (axis cs:8.6,0) rectangle (axis cs:9.4,81.4233333333333);
\draw[draw=none,fill=color0] (axis cs:9.6,0) rectangle (axis cs:10.4,81.77);
\draw[draw=none,fill=color0] (axis cs:10.6,0) rectangle (axis cs:11.4,82.03);
\draw[draw=none,fill=color0] (axis cs:11.6,0) rectangle (axis cs:12.4,82.0566666666667);
\draw[draw=none,fill=color0] (axis cs:12.6,0) rectangle (axis cs:13.4,81.9933333333333);
\draw[draw=none,fill=color0] (axis cs:13.6,0) rectangle (axis cs:14.4,82.0466666666667);
\draw[draw=none,fill=color0] (axis cs:14.6,0) rectangle (axis cs:15.4,81.7833333333333);
\draw[draw=none,fill=color0] (axis cs:15.6,0) rectangle (axis cs:16.4,82.1366666666667);
\draw[draw=none,fill=color0] (axis cs:16.6,0) rectangle (axis cs:17.4,81.91);
\draw[draw=none,fill=color0] (axis cs:17.6,0) rectangle (axis cs:18.4,81.68);
\draw[draw=none,fill=color0] (axis cs:18.6,0) rectangle (axis cs:19.4,81.68);
\draw[draw=none,fill=color0] (axis cs:19.6,0) rectangle (axis cs:20.4,81.3833333333333);
\draw[draw=none,fill=color0] (axis cs:20.6,0) rectangle (axis cs:21.4,81.5033333333333);
\draw[draw=none,fill=color0] (axis cs:21.6,0) rectangle (axis cs:22.4,81.3);
\draw[draw=none,fill=color0] (axis cs:22.6,0) rectangle (axis cs:23.4,81.1333333333333);
\draw[draw=none,fill=color0] (axis cs:23.6,0) rectangle (axis cs:24.4,81.96);
\draw[draw=none,fill=color0] (axis cs:24.6,0) rectangle (axis cs:25.4,81.4966666666667);
\draw[draw=none,fill=color0] (axis cs:25.6,0) rectangle (axis cs:26.4,81.18);
\end{axis}

\end{tikzpicture}


==> images/searchplot_old2.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}%[thick,scale=1.15]
\scriptsize
%\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
%\definecolor{color0}{rgb}{0.19, 0.55, 0.91}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\tikzset{barstyle/.style={draw=none,fill=orange!50}}
\tikzset{incbarstyle/.style={draw=none,fill=caribbeangreen!50}}
\pgfplotsset{%
    width=0.52\textwidth,
    height=.4\textwidth
}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-1.74, xmax=27.74,
xtick style={draw=none},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26},
xticklabel style = {rotate=90.0},
xticklabels={auto\_contrast,equalize,brightness,posterize,translate\_y,color,contrast,detail,flip\_lr,translate\_x,sharpen,solarize,sharpness,cutout,shear\_y,edge\_enhance,crop\_bilinear,shear\_x,contour,invert,min\_,median,max\_,rotate,flip\_ud,blur,gaussian},
y grid style={white!69.0196078431373!black},
ymin=80.5, ymax=82.3,
ytick style={color=black}
]

\draw[incbarstyle] (axis cs:-0.4,0) rectangle (axis cs:0.4,80.7933333333333);
\draw[incbarstyle] (axis cs:0.6,0) rectangle (axis cs:1.4,81.0566666666667);
\draw[incbarstyle] (axis cs:1.6,0) rectangle (axis cs:2.4,81.1833333333333);
\draw[barstyle] (axis cs:2.6,0) rectangle (axis cs:3.4,80.9);
\draw[incbarstyle] (axis cs:3.6,0) rectangle (axis cs:4.4,81.12);
\draw[incbarstyle] (axis cs:4.6,0) rectangle (axis cs:5.4,81.6);
\draw[barstyle] (axis cs:5.6,0) rectangle (axis cs:6.4,81.2166666666667);
\draw[incbarstyle] (axis cs:6.6,0) rectangle (axis cs:7.4,81.39);
\draw[barstyle] (axis cs:7.6,0) rectangle (axis cs:8.4,81.3366666666667);
\draw[incbarstyle] (axis cs:8.6,0) rectangle (axis cs:9.4,81.4233333333333);
\draw[incbarstyle] (axis cs:9.6,0) rectangle (axis cs:10.4,81.77);
\draw[incbarstyle] (axis cs:10.6,0) rectangle (axis cs:11.4,82.03);
\draw[incbarstyle] (axis cs:11.6,0) rectangle (axis cs:12.4,82.0566666666667);
\draw[barstyle] (axis cs:12.6,0) rectangle (axis cs:13.4,81.9933333333333);
\draw[incbarstyle] (axis cs:13.6,0) rectangle (axis cs:14.4,82.0466666666667);
\draw[barstyle] (axis cs:14.6,0) rectangle (axis cs:15.4,81.7833333333333);
\draw[incbarstyle] (axis cs:15.6,0) rectangle (axis cs:16.4,82.1366666666667);
\draw[barstyle] (axis cs:16.6,0) rectangle (axis cs:17.4,81.91);
\draw[barstyle] (axis cs:17.6,0) rectangle (axis cs:18.4,81.68);
\draw[barstyle] (axis cs:18.6,0) rectangle (axis cs:19.4,81.68);
\draw[barstyle] (axis cs:19.6,0) rectangle (axis cs:20.4,81.3833333333333);
\draw[barstyle] (axis cs:20.6,0) rectangle (axis cs:21.4,81.5033333333333);
\draw[barstyle] (axis cs:21.6,0) rectangle (axis cs:22.4,81.3);
\draw[barstyle] (axis cs:22.6,0) rectangle (axis cs:23.4,81.1333333333333);
\draw[barstyle] (axis cs:23.6,0) rectangle (axis cs:24.4,81.96);
\draw[barstyle] (axis cs:24.6,0) rectangle (axis cs:25.4,81.4966666666667);
\draw[barstyle] (axis cs:25.6,0) rectangle (axis cs:26.4,81.18);
\end{axis}

\end{tikzpicture}


==> original_readme.tex <==



% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021. Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.




%%%%%%%%% BODY TEXT
\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the ICCV 2021 web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for ICCV 2021.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\iccvfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a tech report for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the tech report as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the ICCV70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.

\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.

Page numbers should be included for review submissions but not for the 
final paper. Review submissions papers should have page numbers in the 
footer with numbers centered and .75 inches (1.905 cm) from the bottom 
of the page and start on the first page with the number 1.

Page numbers will be added by the publisher to all camera-ready papers 
prior to including them in the proceedings and before submitting the 
papers to IEEE Xplore. As such, your camera-ready submission should 
not include any page numbers. Page numbers should automatically be 
removed by uncommenting (if it's not already) the line
\begin{verbatim}
% \iccvfinalcopy
\end{verbatim}
near the beginning of the .tex file.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centered.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}

%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the ICCV 2021 web page for a discussion
of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.



==> performancepercomputecifar100.tex <==
% This is the CIFAR-10 plot that was in the initial submission
%\begin{document}
\begin{tikzpicture}
\pgfplotsset{
        % initialize Dark2
        cycle list/Dark2,
        % combine it with 'mark list*':
        cycle multiindex* list={
            [3 of]mark list\nextlist
            Dark2\nextlist
        },
    }
\small
\begin{axis}[
    xmode=log,
    log ticks with fixed point,
    % for log axes, x filter operates on LOGS.
    % and log(x * 1000) = log(x) + log(1000):
    %x filter/.code=\pgfmathparse{#1 + 6.90775527898214},
    xlabel=GPU hours (logrithmic axis),
    ylabel=Accuracy (\%),
    width=.5\textwidth,height=.4\textwidth,
    legend columns=2,
    %legend pos=south east,
    legend style={at={(0.325,0.045)},anchor=south west},
    ytick={96,97,98},
    %colorbrewer cycle list=Dark2
    %cycle list name=exotic
    %cycle multi list={Set1-4}
]

% AA 1.45*1/10*12/20*15000 = 1'305
\addplot+[only marks] table{
1602 96.3
1606 97.4
1641 98.0
};
\addlegendentry{AA};



% FAA assume 1x search
\addplot+ table {
4.4 96.4
11.2 97.3
83 98.0
};
\addlegendentry{Fast AA};

% RA
\addplot+ table {
4 95.8
25.25 97.3
166 98
};
\addlegendentry{RA};

% OHL factor=1.5*8=12
\addplot+[only marks] table {
67.2 97.39 
};
\addlegendentry{OHL}

% UA (small WRN, WRN, Shake)
\addplot+[only marks] table {
2.2 96.25
5.6 97.33
41.5 98.10
};
\addlegendentry{UA}


% Adv. AA
\addplot+[only marks] table {
44.8 98.1
111 98.15
};
\addlegendentry{\advaa{} x8}

% AWS factor=(200*4/5+500*10*4/5+300)=6860
\addplot+[only marks] table {
125.4 98.05
};
\addlegendentry{AWS}



% TA
\addplot+[mark=*,color=blue!80] table {
2.2 96.62
5.6 97.46
41.5 98.05
};
\addlegendentry{TA}

% TA w. 8-times batch
\addplot+[color=blue!80] table {
44.8 98.04
111 98.12
};
\addlegendentry{TA x8}

\end{axis}
\end{tikzpicture}
%\end{document}

==> rebuttal/best_param_scaling.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}
\tiny
\definecolor{color0}{rgb}{0.76748424,0.09213602,0.32390525}
\definecolor{color1}{rgb}{0.36196644,0.1195413,0.31852037}
\definecolor{color2}{rgb}{0.25724602,0.10715148,0.27071569}
\definecolor{color3}{rgb}{0.8985026,0.22463251,0.25108745}
\definecolor{color4}{rgb}{0.53726173,0.11587369,0.35642903}
\definecolor{color5}{rgb}{0.47769736,0.12069864,0.34902273}
\definecolor{color6}{rgb}{0.01060815,0.01808215,0.10018654}
\definecolor{color7}{rgb}{0.93899289,0.35250734,0.25452808}
\definecolor{color8}{rgb}{0.81820481,0.12080606,0.29926105}
\definecolor{color9}{rgb}{0.71108138,0.08761223,0.3430635}
\definecolor{color10}{rgb}{0.05032105,0.03936808,0.13020508}
\definecolor{color11}{rgb}{0.95569679,0.48489115,0.33421404}
\definecolor{color12}{rgb}{0.96276513,0.60612062,0.44471698}
\definecolor{color13}{rgb}{0.97564391,0.87403763,0.79725261}
\definecolor{color14}{rgb}{0.86196552,0.16801239,0.27346473}
\definecolor{color15}{rgb}{0.98137749,0.92061729,0.86536915}
\definecolor{color16}{rgb}{0.96709183,0.76855969,0.64207921}
\definecolor{color17}{rgb}{0.94914549,0.42038251,0.28780969}
\definecolor{color18}{rgb}{0.96417332,0.65758729,0.50046894}
\definecolor{color19}{rgb}{0.96004345,0.54657593,0.3870292}
\definecolor{color20}{rgb}{0.96530224,0.71394212,0.56849894}
\definecolor{color21}{rgb}{0.92223947,0.28287251,0.24229568}
\definecolor{color22}{rgb}{0.97071849,0.82151775,0.71987163}
\definecolor{color23}{rgb}{0.65154562,0.09680192,0.35454107}
\definecolor{color24}{rgb}{0.59770215,0.10693774,0.35838029}
\definecolor{color25}{rgb}{0.41925278,0.12173833,0.33640407}
\definecolor{color26}{rgb}{0.10132312,0.06286782,0.16604287}
\definecolor{color27}{rgb}{0.30592213,0.11432553,0.29542718}
\definecolor{color28}{rgb}{0.20388117,0.09608689,0.23860907}
\definecolor{color29}{rgb}{0.15201338,0.08159108,0.20270523}

\begin{axis}[
axis line style={white!15!black},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel={Epochs},
xmin=0, xmax=4,
xtick style={color=white!15!black},
xtick={0.5,1.5,2.5,3.5},
xticklabels={10,25,50,100},
y grid style={white!80!black},
ylabel={Max. strength $M$},
ymin=0, ymax=30,
ytick style={color=white!15!black},
width=\textwidth, height=\textwidth
]
\path [fill=color0, ultra thin]
(axis cs:0,0)
--(axis cs:0,1)
--(axis cs:1,1)
--(axis cs:1,0)
--(axis cs:0,0)
--cycle;
\path [fill=color1, ultra thin]
(axis cs:1,0)
--(axis cs:1,1)
--(axis cs:2,1)
--(axis cs:2,0)
--(axis cs:1,0)
--cycle;
\path [fill=color2, ultra thin]
(axis cs:2,0)
--(axis cs:2,1)
--(axis cs:3,1)
--(axis cs:3,0)
--(axis cs:2,0)
--cycle;
\path [fill=color2, ultra thin]
(axis cs:3,0)
--(axis cs:3,1)
--(axis cs:4,1)
--(axis cs:4,0)
--(axis cs:3,0)
--cycle;
\path [fill=color3, ultra thin]
(axis cs:0,1)
--(axis cs:0,2)
--(axis cs:1,2)
--(axis cs:1,1)
--(axis cs:0,1)
--cycle;
\path [fill=color4, ultra thin]
(axis cs:1,1)
--(axis cs:1,2)
--(axis cs:2,2)
--(axis cs:2,1)
--(axis cs:1,1)
--cycle;
\path [fill=color5, ultra thin]
(axis cs:2,1)
--(axis cs:2,2)
--(axis cs:3,2)
--(axis cs:3,1)
--(axis cs:2,1)
--cycle;
\path [fill=color6, ultra thin]
(axis cs:3,1)
--(axis cs:3,2)
--(axis cs:4,2)
--(axis cs:4,1)
--(axis cs:3,1)
--cycle;
\path [fill=color7, ultra thin]
(axis cs:0,2)
--(axis cs:0,3)
--(axis cs:1,3)
--(axis cs:1,2)
--(axis cs:0,2)
--cycle;
\path [fill=color8, ultra thin]
(axis cs:1,2)
--(axis cs:1,3)
--(axis cs:2,3)
--(axis cs:2,2)
--(axis cs:1,2)
--cycle;
\path [fill=color9, ultra thin]
(axis cs:2,2)
--(axis cs:2,3)
--(axis cs:3,3)
--(axis cs:3,2)
--(axis cs:2,2)
--cycle;
\path [fill=color10, ultra thin]
(axis cs:3,2)
--(axis cs:3,3)
--(axis cs:4,3)
--(axis cs:4,2)
--(axis cs:3,2)
--cycle;
\path [fill=color11, ultra thin]
(axis cs:0,3)
--(axis cs:0,4)
--(axis cs:1,4)
--(axis cs:1,3)
--(axis cs:0,3)
--cycle;
\path [fill=color12, ultra thin]
(axis cs:1,3)
--(axis cs:1,4)
--(axis cs:2,4)
--(axis cs:2,3)
--(axis cs:1,3)
--cycle;
\path [fill=color13, ultra thin]
(axis cs:2,3)
--(axis cs:2,4)
--(axis cs:3,4)
--(axis cs:3,3)
--(axis cs:2,3)
--cycle;
\path [fill=color3, ultra thin]
(axis cs:3,3)
--(axis cs:3,4)
--(axis cs:4,4)
--(axis cs:4,3)
--(axis cs:3,3)
--cycle;
\path [fill=color13, ultra thin]
(axis cs:0,4)
--(axis cs:0,5)
--(axis cs:1,5)
--(axis cs:1,4)
--(axis cs:0,4)
--cycle;
\path [fill=color0, ultra thin]
(axis cs:1,4)
--(axis cs:1,5)
--(axis cs:2,5)
--(axis cs:2,4)
--(axis cs:1,4)
--cycle;
\path [fill=color14, ultra thin]
(axis cs:2,4)
--(axis cs:2,5)
--(axis cs:3,5)
--(axis cs:3,4)
--(axis cs:2,4)
--cycle;
\path [fill=color5, ultra thin]
(axis cs:3,4)
--(axis cs:3,5)
--(axis cs:4,5)
--(axis cs:4,4)
--(axis cs:3,4)
--cycle;
\path [fill=color15, ultra thin]
(axis cs:0,5)
--(axis cs:0,6)
--(axis cs:1,6)
--(axis cs:1,5)
--(axis cs:0,5)
--cycle;
\path [fill=color7, ultra thin]
(axis cs:1,5)
--(axis cs:1,6)
--(axis cs:2,6)
--(axis cs:2,5)
--(axis cs:1,5)
--cycle;
\path [fill=color16, ultra thin]
(axis cs:2,5)
--(axis cs:2,6)
--(axis cs:3,6)
--(axis cs:3,5)
--(axis cs:2,5)
--cycle;
\path [fill=color11, ultra thin]
(axis cs:3,5)
--(axis cs:3,6)
--(axis cs:4,6)
--(axis cs:4,5)
--(axis cs:3,5)
--cycle;
\path [fill=color17, ultra thin]
(axis cs:0,6)
--(axis cs:0,7)
--(axis cs:1,7)
--(axis cs:1,6)
--(axis cs:0,6)
--cycle;
\path [fill=color18, ultra thin]
(axis cs:1,6)
--(axis cs:1,7)
--(axis cs:2,7)
--(axis cs:2,6)
--(axis cs:1,6)
--cycle;
\path [fill=color17, ultra thin]
(axis cs:2,6)
--(axis cs:2,7)
--(axis cs:3,7)
--(axis cs:3,6)
--(axis cs:2,6)
--cycle;
\path [fill=color18, ultra thin]
(axis cs:3,6)
--(axis cs:3,7)
--(axis cs:4,7)
--(axis cs:4,6)
--(axis cs:3,6)
--cycle;
\path [fill=color19, ultra thin]
(axis cs:0,7)
--(axis cs:0,8)
--(axis cs:1,8)
--(axis cs:1,7)
--(axis cs:0,7)
--cycle;
\path [fill=color11, ultra thin]
(axis cs:1,7)
--(axis cs:1,8)
--(axis cs:2,8)
--(axis cs:2,7)
--(axis cs:1,7)
--cycle;
\path [fill=color7, ultra thin]
(axis cs:2,7)
--(axis cs:2,8)
--(axis cs:3,8)
--(axis cs:3,7)
--(axis cs:2,7)
--cycle;
\path [fill=color17, ultra thin]
(axis cs:3,7)
--(axis cs:3,8)
--(axis cs:4,8)
--(axis cs:4,7)
--(axis cs:3,7)
--cycle;
\path [fill=color20, ultra thin]
(axis cs:0,8)
--(axis cs:0,9)
--(axis cs:1,9)
--(axis cs:1,8)
--(axis cs:0,8)
--cycle;
\path [fill=color15, ultra thin]
(axis cs:1,8)
--(axis cs:1,9)
--(axis cs:2,9)
--(axis cs:2,8)
--(axis cs:1,8)
--cycle;
\path [fill=color21, ultra thin]
(axis cs:2,8)
--(axis cs:2,9)
--(axis cs:3,9)
--(axis cs:3,8)
--(axis cs:2,8)
--cycle;
\path [fill=color20, ultra thin]
(axis cs:3,8)
--(axis cs:3,9)
--(axis cs:4,9)
--(axis cs:4,8)
--(axis cs:3,8)
--cycle;
\path [fill=color16, ultra thin]
(axis cs:0,9)
--(axis cs:0,10)
--(axis cs:1,10)
--(axis cs:1,9)
--(axis cs:0,9)
--cycle;
\path [fill=color13, ultra thin]
(axis cs:1,9)
--(axis cs:1,10)
--(axis cs:2,10)
--(axis cs:2,9)
--(axis cs:1,9)
--cycle;
\path [fill=color18, ultra thin]
(axis cs:2,9)
--(axis cs:2,10)
--(axis cs:3,10)
--(axis cs:3,9)
--(axis cs:2,9)
--cycle;
\path [fill=color16, ultra thin]
(axis cs:3,9)
--(axis cs:3,10)
--(axis cs:4,10)
--(axis cs:4,9)
--(axis cs:3,9)
--cycle;
\path [fill=color18, ultra thin]
(axis cs:0,10)
--(axis cs:0,11)
--(axis cs:1,11)
--(axis cs:1,10)
--(axis cs:0,10)
--cycle;
\path [fill=color20, ultra thin]
(axis cs:1,10)
--(axis cs:1,11)
--(axis cs:2,11)
--(axis cs:2,10)
--(axis cs:1,10)
--cycle;
\path [fill=color12, ultra thin]
(axis cs:2,10)
--(axis cs:2,11)
--(axis cs:3,11)
--(axis cs:3,10)
--(axis cs:2,10)
--cycle;
\path [fill=color12, ultra thin]
(axis cs:3,10)
--(axis cs:3,11)
--(axis cs:4,11)
--(axis cs:4,10)
--(axis cs:3,10)
--cycle;
\path [fill=color22, ultra thin]
(axis cs:0,11)
--(axis cs:0,12)
--(axis cs:1,12)
--(axis cs:1,11)
--(axis cs:0,11)
--cycle;
\path [fill=color22, ultra thin]
(axis cs:1,11)
--(axis cs:1,12)
--(axis cs:2,12)
--(axis cs:2,11)
--(axis cs:1,11)
--cycle;
\path [fill=color22, ultra thin]
(axis cs:2,11)
--(axis cs:2,12)
--(axis cs:3,12)
--(axis cs:3,11)
--(axis cs:2,11)
--cycle;
\path [fill=color22, ultra thin]
(axis cs:3,11)
--(axis cs:3,12)
--(axis cs:4,12)
--(axis cs:4,11)
--(axis cs:3,11)
--cycle;
\path [fill=color12, ultra thin]
(axis cs:0,12)
--(axis cs:0,13)
--(axis cs:1,13)
--(axis cs:1,12)
--(axis cs:0,12)
--cycle;
\path [fill=color16, ultra thin]
(axis cs:1,12)
--(axis cs:1,13)
--(axis cs:2,13)
--(axis cs:2,12)
--(axis cs:1,12)
--cycle;
\path [fill=color15, ultra thin]
(axis cs:2,12)
--(axis cs:2,13)
--(axis cs:3,13)
--(axis cs:3,12)
--(axis cs:2,12)
--cycle;
\path [fill=color21, ultra thin]
(axis cs:3,12)
--(axis cs:3,13)
--(axis cs:4,13)
--(axis cs:4,12)
--(axis cs:3,12)
--cycle;
\path [fill=color14, ultra thin]
(axis cs:0,13)
--(axis cs:0,14)
--(axis cs:1,14)
--(axis cs:1,13)
--(axis cs:0,13)
--cycle;
\path [fill=color3, ultra thin]
(axis cs:1,13)
--(axis cs:1,14)
--(axis cs:2,14)
--(axis cs:2,13)
--(axis cs:1,13)
--cycle;
\path [fill=color11, ultra thin]
(axis cs:2,13)
--(axis cs:2,14)
--(axis cs:3,14)
--(axis cs:3,13)
--(axis cs:2,13)
--cycle;
\path [fill=color15, ultra thin]
(axis cs:3,13)
--(axis cs:3,14)
--(axis cs:4,14)
--(axis cs:4,13)
--(axis cs:3,13)
--cycle;
\path [fill=color21, ultra thin]
(axis cs:0,14)
--(axis cs:0,15)
--(axis cs:1,15)
--(axis cs:1,14)
--(axis cs:0,14)
--cycle;
\path [fill=color19, ultra thin]
(axis cs:1,14)
--(axis cs:1,15)
--(axis cs:2,15)
--(axis cs:2,14)
--(axis cs:1,14)
--cycle;
\path [fill=color20, ultra thin]
(axis cs:2,14)
--(axis cs:2,15)
--(axis cs:3,15)
--(axis cs:3,14)
--(axis cs:2,14)
--cycle;
\path [fill=color13, ultra thin]
(axis cs:3,14)
--(axis cs:3,15)
--(axis cs:4,15)
--(axis cs:4,14)
--(axis cs:3,14)
--cycle;
\path [fill=color8, ultra thin]
(axis cs:0,15)
--(axis cs:0,16)
--(axis cs:1,16)
--(axis cs:1,15)
--(axis cs:0,15)
--cycle;
\path [fill=color14, ultra thin]
(axis cs:1,15)
--(axis cs:1,16)
--(axis cs:2,16)
--(axis cs:2,15)
--(axis cs:1,15)
--cycle;
\path [fill=color3, ultra thin]
(axis cs:2,15)
--(axis cs:2,16)
--(axis cs:3,16)
--(axis cs:3,15)
--(axis cs:2,15)
--cycle;
\path [fill=color19, ultra thin]
(axis cs:3,15)
--(axis cs:3,16)
--(axis cs:4,16)
--(axis cs:4,15)
--(axis cs:3,15)
--cycle;
\path [fill=color9, ultra thin]
(axis cs:0,16)
--(axis cs:0,17)
--(axis cs:1,17)
--(axis cs:1,16)
--(axis cs:0,16)
--cycle;
\path [fill=color23, ultra thin]
(axis cs:1,16)
--(axis cs:1,17)
--(axis cs:2,17)
--(axis cs:2,16)
--(axis cs:1,16)
--cycle;
\path [fill=color8, ultra thin]
(axis cs:2,16)
--(axis cs:2,17)
--(axis cs:3,17)
--(axis cs:3,16)
--(axis cs:2,16)
--cycle;
\path [fill=color14, ultra thin]
(axis cs:3,16)
--(axis cs:3,17)
--(axis cs:4,17)
--(axis cs:4,16)
--(axis cs:3,16)
--cycle;
\path [fill=color24, ultra thin]
(axis cs:0,17)
--(axis cs:0,18)
--(axis cs:1,18)
--(axis cs:1,17)
--(axis cs:0,17)
--cycle;
\path [fill=color17, ultra thin]
(axis cs:1,17)
--(axis cs:1,18)
--(axis cs:2,18)
--(axis cs:2,17)
--(axis cs:1,17)
--cycle;
\path [fill=color19, ultra thin]
(axis cs:2,17)
--(axis cs:2,18)
--(axis cs:3,18)
--(axis cs:3,17)
--(axis cs:2,17)
--cycle;
\path [fill=color8, ultra thin]
(axis cs:3,17)
--(axis cs:3,18)
--(axis cs:4,18)
--(axis cs:4,17)
--(axis cs:3,17)
--cycle;
\path [fill=color23, ultra thin]
(axis cs:0,18)
--(axis cs:0,19)
--(axis cs:1,19)
--(axis cs:1,18)
--(axis cs:0,18)
--cycle;
\path [fill=color21, ultra thin]
(axis cs:1,18)
--(axis cs:1,19)
--(axis cs:2,19)
--(axis cs:2,18)
--(axis cs:1,18)
--cycle;
\path [fill=color0, ultra thin]
(axis cs:2,18)
--(axis cs:2,19)
--(axis cs:3,19)
--(axis cs:3,18)
--(axis cs:2,18)
--cycle;
\path [fill=color24, ultra thin]
(axis cs:3,18)
--(axis cs:3,19)
--(axis cs:4,19)
--(axis cs:4,18)
--(axis cs:3,18)
--cycle;
\path [fill=color4, ultra thin]
(axis cs:0,19)
--(axis cs:0,20)
--(axis cs:1,20)
--(axis cs:1,19)
--(axis cs:0,19)
--cycle;
\path [fill=color24, ultra thin]
(axis cs:1,19)
--(axis cs:1,20)
--(axis cs:2,20)
--(axis cs:2,19)
--(axis cs:1,19)
--cycle;
\path [fill=color23, ultra thin]
(axis cs:2,19)
--(axis cs:2,20)
--(axis cs:3,20)
--(axis cs:3,19)
--(axis cs:2,19)
--cycle;
\path [fill=color9, ultra thin]
(axis cs:3,19)
--(axis cs:3,20)
--(axis cs:4,20)
--(axis cs:4,19)
--(axis cs:3,19)
--cycle;
\path [fill=color5, ultra thin]
(axis cs:0,20)
--(axis cs:0,21)
--(axis cs:1,21)
--(axis cs:1,20)
--(axis cs:0,20)
--cycle;
\path [fill=color9, ultra thin]
(axis cs:1,20)
--(axis cs:1,21)
--(axis cs:2,21)
--(axis cs:2,20)
--(axis cs:1,20)
--cycle;
\path [fill=color25, ultra thin]
(axis cs:2,20)
--(axis cs:2,21)
--(axis cs:3,21)
--(axis cs:3,20)
--(axis cs:2,20)
--cycle;
\path [fill=color7, ultra thin]
(axis cs:3,20)
--(axis cs:3,21)
--(axis cs:4,21)
--(axis cs:4,20)
--(axis cs:3,20)
--cycle;
\path [fill=color25, ultra thin]
(axis cs:0,21)
--(axis cs:0,22)
--(axis cs:1,22)
--(axis cs:1,21)
--(axis cs:0,21)
--cycle;
\path [fill=color25, ultra thin]
(axis cs:1,21)
--(axis cs:1,22)
--(axis cs:2,22)
--(axis cs:2,21)
--(axis cs:1,21)
--cycle;
\path [fill=color1, ultra thin]
(axis cs:2,21)
--(axis cs:2,22)
--(axis cs:3,22)
--(axis cs:3,21)
--(axis cs:2,21)
--cycle;
\path [fill=color26, ultra thin]
(axis cs:3,21)
--(axis cs:3,22)
--(axis cs:4,22)
--(axis cs:4,21)
--(axis cs:3,21)
--cycle;
\path [fill=color2, ultra thin]
(axis cs:0,22)
--(axis cs:0,23)
--(axis cs:1,23)
--(axis cs:1,22)
--(axis cs:0,22)
--cycle;
\path [fill=color5, ultra thin]
(axis cs:1,22)
--(axis cs:1,23)
--(axis cs:2,23)
--(axis cs:2,22)
--(axis cs:1,22)
--cycle;
\path [fill=color4, ultra thin]
(axis cs:2,22)
--(axis cs:2,23)
--(axis cs:3,23)
--(axis cs:3,22)
--(axis cs:2,22)
--cycle;
\path [fill=color4, ultra thin]
(axis cs:3,22)
--(axis cs:3,23)
--(axis cs:4,23)
--(axis cs:4,22)
--(axis cs:3,22)
--cycle;
\path [fill=color27, ultra thin]
(axis cs:0,23)
--(axis cs:0,24)
--(axis cs:1,24)
--(axis cs:1,23)
--(axis cs:0,23)
--cycle;
\path [fill=color27, ultra thin]
(axis cs:1,23)
--(axis cs:1,24)
--(axis cs:2,24)
--(axis cs:2,23)
--(axis cs:1,23)
--cycle;
\path [fill=color27, ultra thin]
(axis cs:2,23)
--(axis cs:2,24)
--(axis cs:3,24)
--(axis cs:3,23)
--(axis cs:2,23)
--cycle;
\path [fill=color0, ultra thin]
(axis cs:3,23)
--(axis cs:3,24)
--(axis cs:4,24)
--(axis cs:4,23)
--(axis cs:3,23)
--cycle;
\path [fill=color28, ultra thin]
(axis cs:0,24)
--(axis cs:0,25)
--(axis cs:1,25)
--(axis cs:1,24)
--(axis cs:0,24)
--cycle;
\path [fill=color28, ultra thin]
(axis cs:1,24)
--(axis cs:1,25)
--(axis cs:2,25)
--(axis cs:2,24)
--(axis cs:1,24)
--cycle;
\path [fill=color26, ultra thin]
(axis cs:2,24)
--(axis cs:2,25)
--(axis cs:3,25)
--(axis cs:3,24)
--(axis cs:2,24)
--cycle;
\path [fill=color23, ultra thin]
(axis cs:3,24)
--(axis cs:3,25)
--(axis cs:4,25)
--(axis cs:4,24)
--(axis cs:3,24)
--cycle;
\path [fill=color1, ultra thin]
(axis cs:0,25)
--(axis cs:0,26)
--(axis cs:1,26)
--(axis cs:1,25)
--(axis cs:0,25)
--cycle;
\path [fill=color2, ultra thin]
(axis cs:1,25)
--(axis cs:1,26)
--(axis cs:2,26)
--(axis cs:2,25)
--(axis cs:1,25)
--cycle;
\path [fill=color24, ultra thin]
(axis cs:2,25)
--(axis cs:2,26)
--(axis cs:3,26)
--(axis cs:3,25)
--(axis cs:2,25)
--cycle;
\path [fill=color1, ultra thin]
(axis cs:3,25)
--(axis cs:3,26)
--(axis cs:4,26)
--(axis cs:4,25)
--(axis cs:3,25)
--cycle;
\path [fill=color29, ultra thin]
(axis cs:0,26)
--(axis cs:0,27)
--(axis cs:1,27)
--(axis cs:1,26)
--(axis cs:0,26)
--cycle;
\path [fill=color29, ultra thin]
(axis cs:1,26)
--(axis cs:1,27)
--(axis cs:2,27)
--(axis cs:2,26)
--(axis cs:1,26)
--cycle;
\path [fill=color6, ultra thin]
(axis cs:2,26)
--(axis cs:2,27)
--(axis cs:3,27)
--(axis cs:3,26)
--(axis cs:2,26)
--cycle;
\path [fill=color25, ultra thin]
(axis cs:3,26)
--(axis cs:3,27)
--(axis cs:4,27)
--(axis cs:4,26)
--(axis cs:3,26)
--cycle;
\path [fill=color10, ultra thin]
(axis cs:0,27)
--(axis cs:0,28)
--(axis cs:1,28)
--(axis cs:1,27)
--(axis cs:0,27)
--cycle;
\path [fill=color6, ultra thin]
(axis cs:1,27)
--(axis cs:1,28)
--(axis cs:2,28)
--(axis cs:2,27)
--(axis cs:1,27)
--cycle;
\path [fill=color29, ultra thin]
(axis cs:2,27)
--(axis cs:2,28)
--(axis cs:3,28)
--(axis cs:3,27)
--(axis cs:2,27)
--cycle;
\path [fill=color28, ultra thin]
(axis cs:3,27)
--(axis cs:3,28)
--(axis cs:4,28)
--(axis cs:4,27)
--(axis cs:3,27)
--cycle;
\path [fill=color6, ultra thin]
(axis cs:0,28)
--(axis cs:0,29)
--(axis cs:1,29)
--(axis cs:1,28)
--(axis cs:0,28)
--cycle;
\path [fill=color26, ultra thin]
(axis cs:1,28)
--(axis cs:1,29)
--(axis cs:2,29)
--(axis cs:2,28)
--(axis cs:1,28)
--cycle;
\path [fill=color10, ultra thin]
(axis cs:2,28)
--(axis cs:2,29)
--(axis cs:3,29)
--(axis cs:3,28)
--(axis cs:2,28)
--cycle;
\path [fill=color29, ultra thin]
(axis cs:3,28)
--(axis cs:3,29)
--(axis cs:4,29)
--(axis cs:4,28)
--(axis cs:3,28)
--cycle;
\path [fill=color26, ultra thin]
(axis cs:0,29)
--(axis cs:0,30)
--(axis cs:1,30)
--(axis cs:1,29)
--(axis cs:0,29)
--cycle;
\path [fill=color10, ultra thin]
(axis cs:1,29)
--(axis cs:1,30)
--(axis cs:2,30)
--(axis cs:2,29)
--(axis cs:1,29)
--cycle;
\path [fill=color28, ultra thin]
(axis cs:2,29)
--(axis cs:2,30)
--(axis cs:3,30)
--(axis cs:3,29)
--(axis cs:2,29)
--cycle;
\path [fill=color27, ultra thin]
(axis cs:3,29)
--(axis cs:3,30)
--(axis cs:4,30)
--(axis cs:4,29)
--(axis cs:3,29)
--cycle;

\end{axis}

\end{tikzpicture}


==> rebuttal/noise_scaling.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}

\tiny
\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, at={(0.5,-.5)},anchor=north},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel={Mean Accuracy},
xmin=0.845411566666666, xmax=0.963941385714286,
xminorgrids,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel={Spearman's $\rho$},
ymin=0, ymax=0.668921298185561,
ytick style={color=white!15!black},
width=\textwidth, height=.75*\textwidth
]
\addplot [line width=0.48pt, color0]
table {%
0.945139333333333 0.201838567547016
0.954984333333333 0.101375977741908
0.958553666666667 0.0733726622331648
};
\addlegendentry{width scaling, strength search}
\addplot [line width=0.48pt, color1]
table {%
0.861450666666667 0.639623772045823
0.923425333333334 0.332577281553789
0.945139333333333 0.201838567547016
0.956607 0.0679758308677345
};
\addlegendentry{epoch scaling, strength search}
\addplot [line width=0.48pt, color2]
table {%
0.850799285714285 0.331738773518531
0.919439285714286 0.26268269813206
0.942827142857143 0.0536732492510703
};
\addlegendentry{epoch scaling, type search}
\addplot [only marks, mark=*, mark size=.5pt, draw=color0, fill=color0, colormap={mymap}{[1pt]
 rgb(0pt)=(0.01060815,0.01808215,0.10018654);
  rgb(1pt)=(0.01428972,0.02048237,0.10374486);
  rgb(2pt)=(0.01831941,0.0229766,0.10738511);
  rgb(3pt)=(0.02275049,0.02554464,0.11108639);
  rgb(4pt)=(0.02759119,0.02818316,0.11483751);
  rgb(5pt)=(0.03285175,0.03088792,0.11863035);
  rgb(6pt)=(0.03853466,0.03365771,0.12245873);
  rgb(7pt)=(0.04447016,0.03648425,0.12631831);
  rgb(8pt)=(0.05032105,0.03936808,0.13020508);
  rgb(9pt)=(0.05611171,0.04224835,0.13411624);
  rgb(10pt)=(0.0618531,0.04504866,0.13804929);
  rgb(11pt)=(0.06755457,0.04778179,0.14200206);
  rgb(12pt)=(0.0732236,0.05045047,0.14597263);
  rgb(13pt)=(0.0788708,0.05305461,0.14995981);
  rgb(14pt)=(0.08450105,0.05559631,0.15396203);
  rgb(15pt)=(0.09011319,0.05808059,0.15797687);
  rgb(16pt)=(0.09572396,0.06050127,0.16200507);
  rgb(17pt)=(0.10132312,0.06286782,0.16604287);
  rgb(18pt)=(0.10692823,0.06517224,0.17009175);
  rgb(19pt)=(0.1125315,0.06742194,0.17414848);
  rgb(20pt)=(0.11813947,0.06961499,0.17821272);
  rgb(21pt)=(0.12375803,0.07174938,0.18228425);
  rgb(22pt)=(0.12938228,0.07383015,0.18636053);
  rgb(23pt)=(0.13501631,0.07585609,0.19044109);
  rgb(24pt)=(0.14066867,0.0778224,0.19452676);
  rgb(25pt)=(0.14633406,0.07973393,0.1986151);
  rgb(26pt)=(0.15201338,0.08159108,0.20270523);
  rgb(27pt)=(0.15770877,0.08339312,0.20679668);
  rgb(28pt)=(0.16342174,0.0851396,0.21088893);
  rgb(29pt)=(0.16915387,0.08682996,0.21498104);
  rgb(30pt)=(0.17489524,0.08848235,0.2190294);
  rgb(31pt)=(0.18065495,0.09009031,0.22303512);
  rgb(32pt)=(0.18643324,0.09165431,0.22699705);
  rgb(33pt)=(0.19223028,0.09317479,0.23091409);
  rgb(34pt)=(0.19804623,0.09465217,0.23478512);
  rgb(35pt)=(0.20388117,0.09608689,0.23860907);
  rgb(36pt)=(0.20973515,0.09747934,0.24238489);
  rgb(37pt)=(0.21560818,0.09882993,0.24611154);
  rgb(38pt)=(0.22150014,0.10013944,0.2497868);
  rgb(39pt)=(0.22741085,0.10140876,0.25340813);
  rgb(40pt)=(0.23334047,0.10263737,0.25697736);
  rgb(41pt)=(0.23928891,0.10382562,0.2604936);
  rgb(42pt)=(0.24525608,0.10497384,0.26395596);
  rgb(43pt)=(0.25124182,0.10608236,0.26736359);
  rgb(44pt)=(0.25724602,0.10715148,0.27071569);
  rgb(45pt)=(0.26326851,0.1081815,0.27401148);
  rgb(46pt)=(0.26930915,0.1091727,0.2772502);
  rgb(47pt)=(0.27536766,0.11012568,0.28043021);
  rgb(48pt)=(0.28144375,0.11104133,0.2835489);
  rgb(49pt)=(0.2875374,0.11191896,0.28660853);
  rgb(50pt)=(0.29364846,0.11275876,0.2896085);
  rgb(51pt)=(0.29977678,0.11356089,0.29254823);
  rgb(52pt)=(0.30592213,0.11432553,0.29542718);
  rgb(53pt)=(0.31208435,0.11505284,0.29824485);
  rgb(54pt)=(0.31826327,0.1157429,0.30100076);
  rgb(55pt)=(0.32445869,0.11639585,0.30369448);
  rgb(56pt)=(0.33067031,0.11701189,0.30632563);
  rgb(57pt)=(0.33689808,0.11759095,0.3088938);
  rgb(58pt)=(0.34314168,0.11813362,0.31139721);
  rgb(59pt)=(0.34940101,0.11863987,0.3138355);
  rgb(60pt)=(0.355676,0.11910909,0.31620996);
  rgb(61pt)=(0.36196644,0.1195413,0.31852037);
  rgb(62pt)=(0.36827206,0.11993653,0.32076656);
  rgb(63pt)=(0.37459292,0.12029443,0.32294825);
  rgb(64pt)=(0.38092887,0.12061482,0.32506528);
  rgb(65pt)=(0.38727975,0.12089756,0.3271175);
  rgb(66pt)=(0.39364518,0.12114272,0.32910494);
  rgb(67pt)=(0.40002537,0.12134964,0.33102734);
  rgb(68pt)=(0.40642019,0.12151801,0.33288464);
  rgb(69pt)=(0.41282936,0.12164769,0.33467689);
  rgb(70pt)=(0.41925278,0.12173833,0.33640407);
  rgb(71pt)=(0.42569057,0.12178916,0.33806605);
  rgb(72pt)=(0.43214263,0.12179973,0.33966284);
  rgb(73pt)=(0.43860848,0.12177004,0.34119475);
  rgb(74pt)=(0.44508855,0.12169883,0.34266151);
  rgb(75pt)=(0.45158266,0.12158557,0.34406324);
  rgb(76pt)=(0.45809049,0.12142996,0.34540024);
  rgb(77pt)=(0.46461238,0.12123063,0.34667231);
  rgb(78pt)=(0.47114798,0.12098721,0.34787978);
  rgb(79pt)=(0.47769736,0.12069864,0.34902273);
  rgb(80pt)=(0.48426077,0.12036349,0.35010104);
  rgb(81pt)=(0.49083761,0.11998161,0.35111537);
  rgb(82pt)=(0.49742847,0.11955087,0.35206533);
  rgb(83pt)=(0.50403286,0.11907081,0.35295152);
  rgb(84pt)=(0.51065109,0.11853959,0.35377385);
  rgb(85pt)=(0.51728314,0.1179558,0.35453252);
  rgb(86pt)=(0.52392883,0.11731817,0.35522789);
  rgb(87pt)=(0.53058853,0.11662445,0.35585982);
  rgb(88pt)=(0.53726173,0.11587369,0.35642903);
  rgb(89pt)=(0.54394898,0.11506307,0.35693521);
  rgb(90pt)=(0.5506426,0.11420757,0.35737863);
  rgb(91pt)=(0.55734473,0.11330456,0.35775059);
  rgb(92pt)=(0.56405586,0.11235265,0.35804813);
  rgb(93pt)=(0.57077365,0.11135597,0.35827146);
  rgb(94pt)=(0.5774991,0.11031233,0.35841679);
  rgb(95pt)=(0.58422945,0.10922707,0.35848469);
  rgb(96pt)=(0.59096382,0.10810205,0.35847347);
  rgb(97pt)=(0.59770215,0.10693774,0.35838029);
  rgb(98pt)=(0.60444226,0.10573912,0.35820487);
  rgb(99pt)=(0.61118304,0.10450943,0.35794557);
  rgb(100pt)=(0.61792306,0.10325288,0.35760108);
  rgb(101pt)=(0.62466162,0.10197244,0.35716891);
  rgb(102pt)=(0.63139686,0.10067417,0.35664819);
  rgb(103pt)=(0.63812122,0.09938212,0.35603757);
  rgb(104pt)=(0.64483795,0.0980891,0.35533555);
  rgb(105pt)=(0.65154562,0.09680192,0.35454107);
  rgb(106pt)=(0.65824241,0.09552918,0.3536529);
  rgb(107pt)=(0.66492652,0.09428017,0.3526697);
  rgb(108pt)=(0.67159578,0.09306598,0.35159077);
  rgb(109pt)=(0.67824099,0.09192342,0.3504148);
  rgb(110pt)=(0.684863,0.09085633,0.34914061);
  rgb(111pt)=(0.69146268,0.0898675,0.34776864);
  rgb(112pt)=(0.69803757,0.08897226,0.3462986);
  rgb(113pt)=(0.70457834,0.0882129,0.34473046);
  rgb(114pt)=(0.71108138,0.08761223,0.3430635);
  rgb(115pt)=(0.7175507,0.08716212,0.34129974);
  rgb(116pt)=(0.72398193,0.08688725,0.33943958);
  rgb(117pt)=(0.73035829,0.0868623,0.33748452);
  rgb(118pt)=(0.73669146,0.08704683,0.33543669);
  rgb(119pt)=(0.74297501,0.08747196,0.33329799);
  rgb(120pt)=(0.74919318,0.08820542,0.33107204);
  rgb(121pt)=(0.75535825,0.08919792,0.32876184);
  rgb(122pt)=(0.76145589,0.09050716,0.32637117);
  rgb(123pt)=(0.76748424,0.09213602,0.32390525);
  rgb(124pt)=(0.77344838,0.09405684,0.32136808);
  rgb(125pt)=(0.77932641,0.09634794,0.31876642);
  rgb(126pt)=(0.78513609,0.09892473,0.31610488);
  rgb(127pt)=(0.79085854,0.10184672,0.313391);
  rgb(128pt)=(0.7965014,0.10506637,0.31063031);
  rgb(129pt)=(0.80205987,0.10858333,0.30783);
  rgb(130pt)=(0.80752799,0.11239964,0.30499738);
  rgb(131pt)=(0.81291606,0.11645784,0.30213802);
  rgb(132pt)=(0.81820481,0.12080606,0.29926105);
  rgb(133pt)=(0.82341472,0.12535343,0.2963705);
  rgb(134pt)=(0.82852822,0.13014118,0.29347474);
  rgb(135pt)=(0.83355779,0.13511035,0.29057852);
  rgb(136pt)=(0.83850183,0.14025098,0.2876878);
  rgb(137pt)=(0.84335441,0.14556683,0.28480819);
  rgb(138pt)=(0.84813096,0.15099892,0.281943);
  rgb(139pt)=(0.85281737,0.15657772,0.27909826);
  rgb(140pt)=(0.85742602,0.1622583,0.27627462);
  rgb(141pt)=(0.86196552,0.16801239,0.27346473);
  rgb(142pt)=(0.86641628,0.17387796,0.27070818);
  rgb(143pt)=(0.87079129,0.17982114,0.26797378);
  rgb(144pt)=(0.87507281,0.18587368,0.26529697);
  rgb(145pt)=(0.87925878,0.19203259,0.26268136);
  rgb(146pt)=(0.8833417,0.19830556,0.26014181);
  rgb(147pt)=(0.88731387,0.20469941,0.25769539);
  rgb(148pt)=(0.89116859,0.21121788,0.2553592);
  rgb(149pt)=(0.89490337,0.21785614,0.25314362);
  rgb(150pt)=(0.8985026,0.22463251,0.25108745);
  rgb(151pt)=(0.90197527,0.23152063,0.24918223);
  rgb(152pt)=(0.90530097,0.23854541,0.24748098);
  rgb(153pt)=(0.90848638,0.24568473,0.24598324);
  rgb(154pt)=(0.911533,0.25292623,0.24470258);
  rgb(155pt)=(0.9144225,0.26028902,0.24369359);
  rgb(156pt)=(0.91717106,0.26773821,0.24294137);
  rgb(157pt)=(0.91978131,0.27526191,0.24245973);
  rgb(158pt)=(0.92223947,0.28287251,0.24229568);
  rgb(159pt)=(0.92456587,0.29053388,0.24242622);
  rgb(160pt)=(0.92676657,0.29823282,0.24285536);
  rgb(161pt)=(0.92882964,0.30598085,0.24362274);
  rgb(162pt)=(0.93078135,0.31373977,0.24468803);
  rgb(163pt)=(0.93262051,0.3215093,0.24606461);
  rgb(164pt)=(0.93435067,0.32928362,0.24775328);
  rgb(165pt)=(0.93599076,0.33703942,0.24972157);
  rgb(166pt)=(0.93752831,0.34479177,0.25199928);
  rgb(167pt)=(0.93899289,0.35250734,0.25452808);
  rgb(168pt)=(0.94036561,0.36020899,0.25734661);
  rgb(169pt)=(0.94167588,0.36786594,0.2603949);
  rgb(170pt)=(0.94291042,0.37549479,0.26369821);
  rgb(171pt)=(0.94408513,0.3830811,0.26722004);
  rgb(172pt)=(0.94520419,0.39062329,0.27094924);
  rgb(173pt)=(0.94625977,0.39813168,0.27489742);
  rgb(174pt)=(0.94727016,0.4055909,0.27902322);
  rgb(175pt)=(0.94823505,0.41300424,0.28332283);
  rgb(176pt)=(0.94914549,0.42038251,0.28780969);
  rgb(177pt)=(0.95001704,0.42771398,0.29244728);
  rgb(178pt)=(0.95085121,0.43500005,0.29722817);
  rgb(179pt)=(0.95165009,0.44224144,0.30214494);
  rgb(180pt)=(0.9524044,0.44944853,0.3072105);
  rgb(181pt)=(0.95312556,0.45661389,0.31239776);
  rgb(182pt)=(0.95381595,0.46373781,0.31769923);
  rgb(183pt)=(0.95447591,0.47082238,0.32310953);
  rgb(184pt)=(0.95510255,0.47787236,0.32862553);
  rgb(185pt)=(0.95569679,0.48489115,0.33421404);
  rgb(186pt)=(0.95626788,0.49187351,0.33985601);
  rgb(187pt)=(0.95681685,0.49882008,0.34555431);
  rgb(188pt)=(0.9573439,0.50573243,0.35130912);
  rgb(189pt)=(0.95784842,0.51261283,0.35711942);
  rgb(190pt)=(0.95833051,0.51946267,0.36298589);
  rgb(191pt)=(0.95879054,0.52628305,0.36890904);
  rgb(192pt)=(0.95922872,0.53307513,0.3748895);
  rgb(193pt)=(0.95964538,0.53983991,0.38092784);
  rgb(194pt)=(0.96004345,0.54657593,0.3870292);
  rgb(195pt)=(0.96042097,0.55328624,0.39319057);
  rgb(196pt)=(0.96077819,0.55997184,0.39941173);
  rgb(197pt)=(0.9611152,0.5666337,0.40569343);
  rgb(198pt)=(0.96143273,0.57327231,0.41203603);
  rgb(199pt)=(0.96173392,0.57988594,0.41844491);
  rgb(200pt)=(0.96201757,0.58647675,0.42491751);
  rgb(201pt)=(0.96228344,0.59304598,0.43145271);
  rgb(202pt)=(0.96253168,0.5995944,0.43805131);
  rgb(203pt)=(0.96276513,0.60612062,0.44471698);
  rgb(204pt)=(0.96298491,0.6126247,0.45145074);
  rgb(205pt)=(0.96318967,0.61910879,0.45824902);
  rgb(206pt)=(0.96337949,0.6255736,0.46511271);
  rgb(207pt)=(0.96355923,0.63201624,0.47204746);
  rgb(208pt)=(0.96372785,0.63843852,0.47905028);
  rgb(209pt)=(0.96388426,0.64484214,0.4861196);
  rgb(210pt)=(0.96403203,0.65122535,0.4932578);
  rgb(211pt)=(0.96417332,0.65758729,0.50046894);
  rgb(212pt)=(0.9643063,0.66393045,0.5077467);
  rgb(213pt)=(0.96443322,0.67025402,0.51509334);
  rgb(214pt)=(0.96455845,0.67655564,0.52251447);
  rgb(215pt)=(0.96467922,0.68283846,0.53000231);
  rgb(216pt)=(0.96479861,0.68910113,0.53756026);
  rgb(217pt)=(0.96492035,0.69534192,0.5451917);
  rgb(218pt)=(0.96504223,0.7015636,0.5528892);
  rgb(219pt)=(0.96516917,0.70776351,0.5606593);
  rgb(220pt)=(0.96530224,0.71394212,0.56849894);
  rgb(221pt)=(0.96544032,0.72010124,0.57640375);
  rgb(222pt)=(0.96559206,0.72623592,0.58438387);
  rgb(223pt)=(0.96575293,0.73235058,0.59242739);
  rgb(224pt)=(0.96592829,0.73844258,0.60053991);
  rgb(225pt)=(0.96612013,0.74451182,0.60871954);
  rgb(226pt)=(0.96632832,0.75055966,0.61696136);
  rgb(227pt)=(0.96656022,0.75658231,0.62527295);
  rgb(228pt)=(0.96681185,0.76258381,0.63364277);
  rgb(229pt)=(0.96709183,0.76855969,0.64207921);
  rgb(230pt)=(0.96739773,0.77451297,0.65057302);
  rgb(231pt)=(0.96773482,0.78044149,0.65912731);
  rgb(232pt)=(0.96810471,0.78634563,0.66773889);
  rgb(233pt)=(0.96850919,0.79222565,0.6764046);
  rgb(234pt)=(0.96893132,0.79809112,0.68512266);
  rgb(235pt)=(0.96935926,0.80395415,0.69383201);
  rgb(236pt)=(0.9698028,0.80981139,0.70252255);
  rgb(237pt)=(0.97025511,0.81566605,0.71120296);
  rgb(238pt)=(0.97071849,0.82151775,0.71987163);
  rgb(239pt)=(0.97120159,0.82736371,0.72851999);
  rgb(240pt)=(0.97169389,0.83320847,0.73716071);
  rgb(241pt)=(0.97220061,0.83905052,0.74578903);
  rgb(242pt)=(0.97272597,0.84488881,0.75440141);
  rgb(243pt)=(0.97327085,0.85072354,0.76299805);
  rgb(244pt)=(0.97383206,0.85655639,0.77158353);
  rgb(245pt)=(0.97441222,0.86238689,0.78015619);
  rgb(246pt)=(0.97501782,0.86821321,0.78871034);
  rgb(247pt)=(0.97564391,0.87403763,0.79725261);
  rgb(248pt)=(0.97628674,0.87986189,0.8057883);
  rgb(249pt)=(0.97696114,0.88568129,0.81430324);
  rgb(250pt)=(0.97765722,0.89149971,0.82280948);
  rgb(251pt)=(0.97837585,0.89731727,0.83130786);
  rgb(252pt)=(0.97912374,0.90313207,0.83979337);
  rgb(253pt)=(0.979891,0.90894778,0.84827858);
  rgb(254pt)=(0.98067764,0.91476465,0.85676611);
  rgb(255pt)=(0.98137749,0.92061729,0.86536915)
}, forget plot]
table{%
x                      y
0.945139333333333 0.201838567547016
0.954984333333333 0.101375977741908
0.958553666666667 0.0733726622331648
0.861450666666667 0.639623772045823
0.923425333333334 0.332577281553789
0.945139333333333 0.201838567547016
0.956607 0.0679758308677345
0.850799285714285 0.331738773518531
0.919439285714286 0.26268269813206
0.942827142857143 0.0536732492510703
};
\end{axis}

\end{tikzpicture}


==> tikzdice.tex <==

% Put this file into the preamble and call it via 
% \input{tikzdice.tex}
%
% Jesse Hamner
% https://github.com/jessehamner/tikzdice
% 2020


\usetikzlibrary{arrows}

\tikzset{
  treenode/.style = {align=center, text centered,
    font=\sffamily},
  arn_n/.style = {treenode, font=\sffamily\bfseries, draw=black,
    fill=black, text width=1.5em},  
  arn_r/.style = {treenode, text width=1.5em},
  arn_x/.style = {treenode, minimum width=0.5em, minimum height=0.5em}
}

\newcommand{\majelaxis}{0.5}
\newcommand{\minelaxis}{0.125}

\newcommand{\headtext}{\color{red}\textbf{H}}

\newcommand{\dieone}{\maindie{1}{0}}
\newcommand{\dietwo}{\maindie{2}{0}}
\newcommand{\diethree}{\maindie{3}{0}}
\newcommand{\diefour}{\maindie{4}{0}}
\newcommand{\diefive}{\maindie{5}{0}}
\newcommand{\diesix}{\maindie{6}{0}}

\newcommand{\pipsize}{3.05pt}
\newcommand{\diecolor}{red}
\newcommand{\pipcolor}{red}
\newcommand{\fieldfill}{white}

\newcommand{\piplocation}[2]{\filldraw[fill=\pipcolor] (#1,#2) circle (\pipsize);}

\newcommand{\piplocationone}{\piplocation{0.25}{0.25}}
\newcommand{\piplocationtwo}{\piplocation{0.50}{0.25}}
\newcommand{\piplocationthree}{\piplocation{0.75}{0.25}}
\newcommand{\piplocationfour}{\piplocation{0.25}{0.50}}
\newcommand{\piplocationfive}{\piplocation{0.50}{0.50}}
\newcommand{\piplocationsix}{\piplocation{0.75}{0.50}}
\newcommand{\piplocationseven}{\piplocation{0.25}{0.75}}
\newcommand{\piplocationeight}{\piplocation{0.50}{0.75}}
\newcommand{\piplocationnine}{\piplocation{0.75}{0.75}}

\newcommand{\spreadsix}{\piplocation{0.20}{0.20}\piplocation{0.20}{0.80}
						\piplocation{0.80}{0.20}\piplocation{0.80}{0.80}
						\piplocation{0.50}{0.20}\piplocation{0.50}{0.80}}

\newcommand{\maindie}[2]{
\ifthenelse{#2 = 0}{\renewcommand{\diecolor}{black}\renewcommand{\pipcolor}{black}\renewcommand{\fieldfill}{white}}{}%
\ifthenelse{#2 = 1}{\renewcommand{\diecolor}{red}\renewcommand{\pipcolor}{red}\renewcommand{\fieldfill}{white}}{}%
\ifthenelse{#2 = 2}{\renewcommand{\diecolor}{blue!60}\renewcommand{\pipcolor}{blue!60}\renewcommand{\fieldfill}{white}}{}%
\ifthenelse{#2 = 3}{\renewcommand{\diecolor}{black}\renewcommand{\pipcolor}{white}\renewcommand{\fieldfill}{black}}{}%
\begin{tikzpicture}
  \draw[very thick, rounded corners, \diecolor, fill=\fieldfill] (0,0) rectangle (1,1);
  \ifthenelse{#1 = 1}{\piplocationfive}{}%  
  \ifthenelse{#1 = 2}{\piplocationone\piplocationnine}{}%
  \ifthenelse{#1 = 3}{\piplocationone\piplocationfive\piplocationnine}{}%
  \ifthenelse{#1 = 4}{\piplocationone\piplocationnine\piplocationthree\piplocationseven}{}%
  \ifthenelse{#1 = 5}{\piplocationone\piplocationnine\piplocationthree\piplocationseven\piplocationfive}{}%
  \ifthenelse{#1 = 6}{\piplocation{0.20}{0.25}\piplocation{0.20}{0.75}
					  \piplocation{0.80}{0.25}\piplocation{0.80}{0.75}
					  \piplocation{0.20}{0.50}\piplocation{0.80}{0.50}}{}%

  \ifthenelse{#1 = 7}{\spreadsix\piplocationfive}{}%	  
  \ifthenelse{#1 = 8}{\spreadsix\piplocation{0.20}{0.50}\piplocation{0.80}{0.50}}{}%	  
  \ifthenelse{#1 = 9}{\spreadsix\piplocation{0.20}{0.50}\piplocation{0.80}{0.50}\piplocationfive}{}%
  \ifthenelse{#1 = 0}{}{}%
%    \ifthenelse{#1 = 0}{\draw[very thick, rounded corners, \diecolor, fill=\diecolor!20] (0,0) rectangle (1,1);}{}%  

\end{tikzpicture}
}


\pgfmathdeclarefunction{addone}{1}{
  \pgfmathparse{#1 + \majelaxis}
}

\pgfmathdeclarefunction{addtwo}{1}{
  \pgfmathparse{#1 + \majelaxis + \majelaxis}
}

\pgfmathdeclarefunction{addspace}{1}{
  \pgfmathparse{#1 + 1.15}
}


\newcommand{\coin}[4]{
  \pgfmathsetmacro{\argthree}{addone(#1)}
  \pgfmathsetmacro{\argtwo}{addtwo(#1)}
  
  \shade[left color=white, right color=black]
    ({\argthree},0mm) ellipse (\majelaxis cm and \minelaxis cm);
  \shade[left color=white, right color=black]
    ({#1},0mm) rectangle (\argtwo cm, 1mm);   

  \draw({\argthree},0.5cm) node[color=blue, above]{#2};

  \draw[fill=#4]({\argthree},1mm) ellipse (\majelaxis cm and \minelaxis cm); 
  \draw ({#1},0mm) arc (180:360:\majelaxis cm and \minelaxis cm);
  \draw({#1},0mm) -- ({#1}, 1mm);
  \draw({\argtwo},0mm) -- ({\argtwo}, 1mm);
  
  \draw({\argthree},-0.4cm) node[color=black, below]{#3};
}

\newcommand{\heads}[2]{
\coin{#1}{#2}{\headtext}{blue!50}
}

\newcommand{\tails}[2]{
\coin{#1}{#2}{{\color{gray!70}T}}{white}
}




\newcommand{\wtf}{\theheadpos & \makecoinrow{} \\}

\newcommand{\whichheads}{1}
\newcounter{num}
\setcounter{num}{1}
\newcounter{headpos}
\setcounter{headpos}{1}
\newcounter{int}
\setcounter{int}{1}


% Row of coins, one head, slot #1.

\newcommand{\makecoinrow}{
  \setcounter{int}{1}

  \begin{tikzpicture}[]
    \newdimen\R
    \R=0cm
    
    \loop
      \ifthenelse{\value{int}=\value{headpos}}{\heads{\R}{}}{\tails{\R}{}} 
      \pgfmathsetmacro{\R}{addspace(\R)}
      \stepcounter{int}
      \ifnum \value{int}<11
    \repeat
  
  \end{tikzpicture}
  
  \smallskip
}



% Definition of circles and square
\def\firstcircle{(0,0) circle (1.5cm)}
\def\secondcircle{(2,0) circle (1.5cm)}
\def\firstsquare{(-1.6,-1.6) rectangle (1.6,1.6)}


\def\missed{\LARGE\textbf{X}}
\def\target{\begin{tikzpicture}
  \draw[ultra thick, black, fill=blue!55] (0,0) circle(1cm);
  \draw[fill=red!70] (0,0) circle(0.73cm);
  \draw[fill=yellow] (0,0) circle(0.35cm) node{\small$\times$};
\end{tikzpicture}}

% Set colors
\colorlet{circle edge}{blue!50}
\colorlet{circle area}{blue!20}
\colorlet{rectangle edge}{blue!50}
\colorlet{rectangle area}{blue!20}

\tikzset{filled/.style={fill=circle area, draw=circle edge, thick},
    	 outline/.style={draw=circle edge, thick}
	    }
\setlength{\parskip}{5mm}





\def\missed{\LARGE\textbf{X}}
\def\target{\begin{tikzpicture}
  \draw[ultra thick, black, fill=blue!55] (0,0) circle(1cm);
  \draw[fill=red!70] (0,0) circle(0.73cm);
  \draw[fill=yellow] (0,0) circle(0.35cm) node{\small$\times$};
\end{tikzpicture}}

\tikzset{
  treenode/.style = {align=center, text centered, font=\sffamily},
  arn_n/.style = {treenode, font=\sffamily\bfseries, draw=black, fill=black},
  arn_r/.style = {treenode},
  arn_x/.style = {treenode}
}

